ChargeX: Exploring State Switching Attack on Electric Vehicle Charging Systems

Electric Vehicle (EV) has become one of the promising solutions to the ever-evolving environmental and energy crisis. The key to the wide adoption of EVs is a pervasive charging infrastructure, composed of both private/home chargers and public/commercial charging stations. The security of EV charging, however, has not been thoroughly investigated. This paper investigates the communication mechanisms between the chargers and EVs, and exposes the lack of protection on the authenticity in the SAE J1772 charging control protocol. To showcase our discoveries, we propose a new class of attacks, ChargeX, which aims to manipulate the charging states or charging rates of EV chargers with the goal of disrupting the charging schedules, causing a denial of service (DoS), or degrading the battery performance. ChargeX inserts a hardware attack circuit to strategically modify the charging control signals. We design and implement multiple attack systems, and evaluate the attacks on a public charging station and two home chargers using a simulated vehicle load in the lab environment. Extensive experiments on different types of chargers demonstrate the effectiveness and generalization of ChargeX. Specifically, we demonstrate that ChargeX can force the switching of an EV's charging state from ``stand by" to ``charging", even when the vehicle is not in the charging state. We further validate the attacks on a Tesla Model 3 vehicle to demonstrate the disruptive impacts of ChargeX. If deployed, ChargeX may significantly demolish people's trust in the EV charging infrastructure.

==> Sections/04AttackOverview.tex <==
\section{\attack Attack Overview}

%In this section, we present an overview of \attack attack, which includes IEMI-based attack and cable tempering attack, whose goals are to manipulate the charging state and charging rate. 

%The IEMI-based attack emits electromagnetic (EM) waves to interfere with the current measurement in the charger control panel. An over-current/reverse-current phenomenon induced by the EM waves will result in the disconnection from the power line. 
%We also propose a cable tempering attack using a hardware circuit design to attach additional components to the charging cable via an extension cable. 
%We mathematically estimate the essential parameters in the attack and leverage the modified cable to achieve the state switching. Here, we propose two hardware manipulation strategies: \emph{serial insertion attack} and \emph{parallel attachment attack}. We further explore an attack automation mechanism to switch the states only when the charger or EV is in a target state 
%launch the state switching attacks that take effect only in the target state, 
%and without any human involvement.
%We further enhance the attack design by enabling automatic parameter adjustment. 
%%Finally, we attempt to manipulate the duty cycle of the control pilot: TLC555-based and fake load-based attack circuits are designed to reduce the duty cycle without affecting normal charging operations. 


%Figure~\ref{fig:overviewIEMI} shows the scenario of IEMI-based attack. The vehicle is being charged by a home EV charger. %One side of the home charger is connected to the socket and the other side is connected to the vehicle.

%We first connect the antenna with the amplifier and then with a EM signal generator. 
%The attacker hide or camouflage the antenna close to the charger control panel, and control the attack frequency and power level far away from the charger using an extension cable connected with a EM signal generator. 
%right above the antenna, e.g., $10cm$, to increase the attack successful rate. 
%During the IEMI attack, the charger will detect the abnormal current in the power line, which will immediately halt the power connection internally with the socket, resulting in a DoS condition. %\ce{undercurrent case}

Figure~\ref{fig:attack_overview} gives an example of \attack. The vehicle is being charged at a public charging station. The red cable represents the malicious J1772 extension cable \cite{extension_cable} in which we embed the attack circuit. Particularly, the attack circuit is placed in the inlet of the extension cable as shown in Figure \ref{fig:extension_cabl}. The attack is covert and difficult to discover without extra caution, as the malicious extension cable can perfectly resemble
that from a legitimate charger. Meanwhile, due to the small size of the attack circuit, it can be completely hidden inside the malicious cable. The connection joint can also be easily hidden, e.g., behind the charging station. 

\begin{figure}[t]
\centering
\includegraphics[width=0.38\textwidth]{figure/overview1-2.pdf}
\caption{\attack attack overview.}
\label{fig:attack_overview}
%\vspace{-16pt}
\end{figure}
